Platform Independent Software Analysis for Near Memory Computing

Near-memory Computing (NMC) promises improved performance for the applications that can exploit the features of emerging memory technologies such as 3D-stacked memory. However, it is not trivial to find such applications and specialized tools are needed to identify them. In this paper, we present PISA-NMC, which extends a state-of-the-art hardware agnostic profiling tool with metrics concerning memory and parallelism, which are relevant for NMC. The metrics include memory entropy, spatial locality, data-level, and basic-block-level parallelism. By profiling a set of representative applications and correlating the metrics with the application's performance on a simulated NMC system, we verify the importance of those metrics. Finally, we demonstrate which metrics are useful in identifying applications suitable for NMC architectures.

==> sections/applicationTable.tex <==
{\scriptsize
\begin{table}[h]

\vspace{-0.2cm}
\centering
\caption{Evaluated applications and their parameters}
\label{tab:results}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{tabular}{p{1cm}p{2.6cm}|p{1.5cm}p{0.4cm}}
\hline
\multicolumn{2}{c|}{\textbf{Applications}}  & \multicolumn{2}{c}{\textbf{Parameter }}    \\ 

 Name& Description& Param. & Values  \\ \hline




atax    & Matrix Transpose \newline and Vector Mult.   & Dimensions    \newline Threads &8000 \newline 32 \\

bfs      & Breadth-first \newline Search                        &  Nodes\newline Weights    \newline Threads    \newline Iterations          &1.0m \newline 4\newline32\newline95 \\

bp    & Back-propagation                & Layer Size  \newline Seed   \newline Threads    \newline Iterations                               &1.1m \newline 5\newline 32\newline 9\\

cholesky   & Cholesky \newline Decomposition                  & Dimensions             \newline Threads  \newline Iterations     &2000 \newline 32 \newline 60  \\

gemver &Vector Multiply \newline and Matrix\newline Addition  & Dimensions        \newline Threads      \newline Iterations           &8000 \newline 32  \newline 60  \\

gesummv  & Scalar, Vector, and \newline Matrix Mult.  & Dimensions       \newline Threads     \newline Iterations &8000 \newline 32 \newline50  \\


grams   & Gram-Schmidt \newline Process                    & Dimension$_i$ \newline Dimension$_j$    \newline Threads                                       &2000 \newline 2000 \newline32  \\

kmeans     & K-Means \newline Clustering          & Data Size     \newline Clusters  \newline Threads      \newline Iterations                          & 819k  \newline 5\newline32\newline 30\\


lu     & LU Decomposition                          & Dimensions      \newline Threads     \newline Iterations   &2000 \newline 32  \newline 2000   \\


mvt     & Matrix Vector \newline Product     &Dimensions          \newline Threads     \newline Iterations &2000 \newline 32   \newline40 \\

syrk     & Symmetric Rank-k \newline Operations              & Dimension$_i$     \newline Dimension$_j$ \newline  Threads                                &2000 \newline 2000 \newline32     \\


trmm      & Triangular Matrix \newline Multiply       & Dimension$_i$\newline Dimension$_j$              \newline Threads        &2000 \newline 2000 \newline32   \\ 
\bottomrule

\end{tabular}

\vspace{-0.4cm}

\end{table}
}

==> sections/backgrounds_OLD.tex <==




This Section provides an overview on background information. First, we describe the LLVM framework on which the tool is based. Then, we present the structure of PISA.

%Background information is provided in the following sub-sections. In particular, we start by describing the LLVM framework on which the tool is based, and then present the structure of PISA.

%In this section we give the basic information on the LLVM Infrastructure on which is based this work. Then it's presented the Tool that we extended and the Benchmark Suite that we analyzed.

\subsection{LLVM Framework}

The LLVM framework is a collection of modular and reusable compiler and toolchain technologies \cite{Lattner:2004:LCF:977395.977673}. The LLVM core uses an intermediate representation (IR) to represent the application code in a generic way. LLVM's IR is generated through a front-end from the application source code. Then, it can be used to perform analyses or optimizations using the \emph{opt} tool. LLVM's IR can be executed through an interpreter or can be translated into a target-specific executable binary.
Fundamental properties of LLVM's IR are: 1) it is independent of the source language and the target architecture; 2) it is a low-level and RISC-like instruction set allowing to have an unlimited number of virtual registers in static single assignment (SSA) form. These features are essential to simulate an ideal machine \cite{bookCA} that consists of a Von-Neumann system with unlimited resources, such as cores, registers, or in other words when the goal is a perfect machine without the traditional hardware limitations.
LLVM's IR has a hierarchical structure: a \emph{module} that represents the application and contains functions and global variables; a \emph{function} that is a set of basic-blocks; a \emph{basic-block} that consists of \emph{instructions} and represents a single entry and single exit section of code.

\subsection{Tool Architecture}
Our goal is to dynamically analyze a wide range of applications to extract helpful metrics relevant for NMC. We extend PISA that uses an instrumented approach. PISA instruments the code with function calls to an external run-time analysis library. 

\begin{figure}[H]
\centering
\includegraphics[width=8.5cm]{images/pisa}
\caption{Overview of the Platform-Independent Software Analysis Tool \cite{Anghel2016}.
\label{fig:pisa}}
\end{figure}

PISA's architecture is shown in \emph{Figure \ref{fig:pisa}}. Initially, application's source code, e.g. C/C++ code, is translated into the LLVM's IR. Then, \emph{mem2reg} optimization is used to obtain the SSA format. This is done by removing \emph{alloca} instructions for non-aliased scalar variables. In this way, these variables are put in virtual registers. PISA exploits the \emph{opt} tool to perform LLVM's IR optimizations and to perform the instrumentation process using an LLVM pass. This process is done by inserting calls to the external analysis library throughout the application's IR.
The last step consists of a linking process that generates a native executable. On running this executable, we can obtain analysis results for specified metrics in JSON format. PISA can extract metrics such as instruction-level parallelism, data reuse distance, instruction mix, etc. %the metrics mentioned in \emph{Table \ref{tab:pisametrics}}.

The analysis reconstructs and analyzes the program's instruction flow. This is possible because the analysis library is aware of the single entry and exit point for each basic-block. All the instructions contained in the basic-block are analyzed using the external library methods. Only when a load/store or a call is encountered the execution is interrupted in order to allow a dynamic analysis. In the case of load/store, the analysis is restarted by an instrumentation function after the load/store instruction. Instead in the case of a call, the current state of the basic-block is saved and then PISA continues analyzing the basic-blocks pointed by the call.


%\emph{Figure \ref{fig:pisa}} shows PISA (Platform-Independent Software Analysis Tool), the point of reference for this work. PISA analyzes the IR flows performing a hardware independent analysis. In the first stage using the \emph{clang} front-end PISA converts the source code (C/C++, Fortran) into the IR format. The \emph{mem2reg} optimization is used to exploit the SSA format. Next, an LLVM pass performs an IR code instrumentation through the \emph{opt} command. The instrumentation process inserts all the external function calls to the analysis library. This library allows to reconstruct and analyze the program's instruction flow. \gagan{"THIS"-WHAT ARE YOU REFERRING TO?ANALYSIS?LIBRARY CALL?}This can be done because the library is aware of the Basic Blocks execution using a single entry point and a single exit point. \gagan{"THIS"AGAIN IT IS CONFUSING}This allows the framework to process the sequence of instructions. When a load/store or a call instruction is encountered then the basic block execution is interrupted. For memory instruction, the framework must update the addresses and then the execution is restored by a next call. Contrariwise during a call, the tool saves the current state and start analyzing the basic blocks pointed by the call.
%Each instruction is analyzed through different \emph{visit} functions for each characterization metric and the data is stored in separate data structures.

A useful feature of PISA is the support of the MPI and OpenMP standards allowing the analysis of multi-threaded and multi-process applications. In multi-threaded applications, PISA analyzes each thread individually, allocating different data structures for each of them and distinguishing them by the thread ID because the address space is shared. For multi-process applications, this is not needed because each process has its private space for data.
The overhead of this tool depends on the analysis performed. On average the execution-time of the instrumented code is increased by two to three orders of magnitude in comparison to the non-instrumented code. On the other hand, since the analysis is target-independent, this has to be performed only once per application and dataset.

\begin{comment}

\begin{table}[!t]
%\renewcommand{\arraystretch}{1.3}
\caption{PISA's metrics}
\label{tab:pisametrics}
\centering
 \scalebox{0.90}{
\begin{tabular}{c|l}
\hline
\bfseries Metric & \bfseries Description\\
\hline
Instruction Mix & Instruction count for each instruction category\\
\hline
Instruction-level parallelism  & Number of instructions that be can run in parallel\\
\hline
Branch entropy & The measure of randomness of branch outcomes\\
\hline
 Data temporal reuse  & Number of unique memory accesses between two\\
 &  accesses to the same location\\
\hline
MPI communications & Data volume exchanged by MPI pairs\\% during the application run\\
\hline
\end{tabular}}
\end{table}

\end{comment}

\begin{comment}
\begin{table}[!t]
\caption{PISA's Metrics}
\label{tab:pisametrics}
\centering
\begin{tabular}{l|l}
\hline
\multicolumn{1}{c|}{\textbf{Metric}} & \multicolumn{1}{c}{\textbf{Description}}                                                                                 \\ \hline
Instruction Mix                      & \begin{tabular}[c]{@{}l@{}}Instruction count for each instruction \\ category\end{tabular}                               \\ \hline
Instruction-level parallelism        & \begin{tabular}[c]{@{}l@{}}Number of instructions that be can \\ run in parallel\end{tabular}                            \\ \hline
Branch entropy                       & \begin{tabular}[c]{@{}l@{}}The measure of randomness of branch \\ outcomes\end{tabular}                                  \\ \hline
Data temporal reuse                  & \begin{tabular}[c]{@{}l@{}}Number of unique memory accesses \\ between two accesses to the same \\ location\end{tabular} \\ \hline
MPI communications                   & Data volume exchanged by MPI pairs                                                                                       \\ \hline
\end{tabular}
\end{table}


\end{comment}

%\begin{itemize}
%\item Instruction mix: Instruction count for each instruction category
%\item Instruction-level parallelism (ILP): Number of instructions that can run in parallel
%\item Branch entropy: The measure of randomness of branch outcomes
%\item Data temporal reuse (DTR): Number of unique memory access between two access to the same memory location
%\item MPI communications: Data exchanged by MPI pairs during the application run
%\end{itemize}












==> sections/backgrounds_SCOPES.tex <==




%This Section provides an overview on background information. First, we describe the tool architecture. Then, we motivate the Benchmarks selected. Related works conclude the section.



%\subsection{LLVM Framework}
%\gaganAdd{
%\subsection{Tool Architecture}
PISA is based on the LLVM Compiler framework.
%The LLVM compiler framework
%This last one
It uses an intermediate representation (IR), which is generated from the application source code using a clang front-end, to represent the application code in a generic way. This IR is independent of the target architecture and has RISC-like instruction set. Therefore, these features can be used to perform application analysis or optimization using the opt tool.
%}
%\gaganRemove{The LLVM framework is a collection of modular and reusable compiler and toolchain technologies \cite{Lattner:2004:LCF:977395.977673}. The LLVM core uses an intermediate representation (IR) to represent the application code in a generic way. LLVM's IR is generated through a front-end from the application source code. Then, it can be used to perform analyses or optimizations using the \emph{opt} tool. LLVM's IR can be executed through an interpreter or can be translated into a target-specific executable binary.
%Fundamental properties of LLVM's IR are: 1) it is independent of the source language and the target architecture; 2) it is a low-level and RISC-like instruction set allowing to have an unlimited number of virtual registers in static single assignment (SSA) form. These features are essential to simulate an ideal machine \cite{bookCA} that consists of a Von-Neumann system with unlimited resources, such as cores, registers, or in other words when the goal is a perfect machine without the traditional hardware limitations.}
LLVM's IR has a hierarchical structure: a \emph{basic-block} that consists of \emph{instructions} and represents a single entry and single exit section of code; a \emph{function} that is a set of basic-blocks; and a \emph{module} that represents the application and contains functions and global variables.

%\subsection{Tool Architecture}
%Our goal is to dynamically analyze a wide range of applications to extract helpful metrics relevant for NMC. We extend PISA that uses an instrumented approach. PISA instruments the code with function calls to an external run-time analysis library. 

\begin{figure}[ht]
\centering
\includegraphics[width=8.5cm]{images/pisa}
\caption{Overview of the Platform-Independent Software Analysis Tool \cite{Anghel2015AnIA}.
\label{fig:pisa}}
\end{figure}

PISA's architecture is shown in \emph{Figure \ref{fig:pisa}}. Initially, the application source code, e.g. C/C++ code, is translated into the LLVM's IR. %Then, \emph{mem2reg} optimization is used to obtain the SSA format.
%This is done by removing \emph{alloca} instructions for non-aliased scalar variables. In this way, these variables are put in virtual registers. 
PISA exploits the \emph{opt} tool to perform LLVM's IR optimizations and to perform the instrumentation process using an LLVM pass. This process is done by inserting calls to the external analysis library throughout the application's IR.
The last step consists of a linking process that generates a native executable. On running this executable, we can obtain analysis results for specified metrics in JSON format. PISA can extract metrics such as instruction mix, branch entropy, data reuse distance, etc.
%the metrics mentioned in \emph{Table \ref{tab:pisametrics}}.

The analysis reconstructs and analyzes the program's instruction flow. This is possible because the analysis library is aware of the single entry and exit point for each basic-block. All the instructions contained in the basic-block are analyzed using the external library methods. %Only when a load/store or a call is encountered the execution is interrupted in order to allow a dynamic analysis. In the case of load/store, the analysis is restarted by an instrumentation function after the load/store instruction. Instead in the case of a call, the current state of the basic-block is saved and then PISA continues analyzing the basic-blocks pointed by the call.
Moreover, PISA supports the MPI and OpenMP standards allowing the analysis of multi-threaded and multi-process applications.
The tool's overhead depends on the analysis performed. On average the execution-time increases by two to three orders of magnitude in comparison to the non-instrumented code. However, since the analysis is target-independent, this has to be performed only once per application and dataset.

%A useful feature of PISA is the support of the MPI and OpenMP standards allowing the analysis of multi-threaded and multi-process applications. In multi-threaded applications, PISA analyzes each thread individually, allocating different data structures for each of them and distinguishing them by the thread ID because the address space is shared. For multi-process applications, this is not needed because each process has its private space for data.
%The overhead of this tool depends on the analysis performed. On average the execution-time of the instrumented code is increased by two to three orders of magnitude in comparison to the non-instrumented code. On the other hand, since the analysis is target-independent, this has to be performed only once per application and dataset.


%\begin{table}[!t]
%\caption{PISA's metrics}
%\label{tab:pisametrics}
%\centering
% \scalebox{0.80}{
%\begin{tabular}{c|l}
%\hline
%\bfseries Metric & \bfseries Description\\
%\hline
%Instruction Mix & Instruction count for each instruction category\\
%\hline
%Instruction-level parallelism  & Number of instructions that be can run %in parallel\\
%\hline
%Branch entropy & The measure of randomness of branch outcomes\\
%\hline
% Data temporal reuse  & Number of unique memory accesses between two\\
% &  accesses to the same location\\
%\hline
%MPI communications & Data volume exchanged by MPI pairs\\% during the %application run\\
%\hline
%\end{tabular}}
%\end{table}

%\subsection{Benchmarks}
%There is a lack of proper benchmarks to evaluate NMC systems and explore the design space. We select a set of applications from two benchmark suites that are representative of the most common kernels and have been used previously in other related studies: Rodinia ~\cite{zhang2014top}
%,7551394,7756764}
%and Polybench~\cite{7756764}:

%\begin{itemize}

%\item Polybench~\cite{pouchet2012polybench} is a collection of a large number of common kernels like matrix multiplication, stencil, covariance, correlation, etc. Each kernel is in a single file, tunable at compile-time. This, makes instrumentation easier.

%\item Rodinia~\cite{5306797} is a benchmark suite for heterogeneous computing. Rodinia workloads cover a wide range of different behaviors which help a developer in building new systems.
%\end{itemize}

%\subsection{Related Work}
%Considerable effort has been already spent in realizing platform independent characterization tools.
%Cabezas \cite{cabezas2012tool} proposed a tool that can extract different features from workloads but has many limitations: the compiler community no longer supports the LLVM interpreter, and the target applications should be single threaded.
%Another tool has been developed by Shao et al. \cite{shao}. It can extract interesting metrics such as memory entropy and branch entropy. However, this tool has some limitations: it is based on the IDJIT IR (just-in-time compilation) that has compatibility problems with OpenMP and MPI, thus being limited to sequential applications.
%The state-of-the-art tool (called PISA) in workload characterization was presented by Anghel et al. \cite{Anghel2015AnIA}. PISA can analyze multi-threaded applications supporting the OpenMP and the MPI standards. PISA can extract the metrics such as instruction mix, branch entropy, data reuse distance, etc.
%showed in \emph{Table \ref{tab:pisametrics}}.
%We extended PISA with metrics directed towards NMC such as memory entropy and spatial locality, data-level and basic-block-level parallelism. %We also showed the relevance of the proposed metrics correlating the analysis results with the performance on an NMC system.








==> sections/introduction_OLD.tex <==
With the demise of Dennard scaling and slowing of Moore's law, computing performance is hitting a plateau \cite{Esmaeilzadeh:2011:DSE:2024723.2000108}. The improvements in memory and processor technology have grown at a different speed, which is infamously termed as the memory wall \cite{Wulf:1995:HMW:216585.216588}. This technological trend has resulted in a situation where the data transfers to and from memory are often much slower than the processing capabilities of processors. This extreme transition has introduced several challenges in the design of future computing ~architecture.

Additionally, in this big-data era, where data is being generated in a massive amount, across multiple domains, it has created a demand for novel memory-centric designs rather than conventional compute-centric designs \cite{overviewpaper}. In traditional compute-centric systems, we have a couple of compute engines with layers of cache memory. Modern big-data workloads, due to highly random access nature, are not able to efficiently exploit the existing cache hierarchy. Hence, they cause huge cache-flush and data retrieval from off-chip main memory~\cite{awan2015performance,awan2016micro}. This off-chip movement can lead to substantial energy consumption and stalling of compute engines which causes severe performance degradation. However, the advancement in technology has enabled us to bring the compute units in the close proximity of data. This paradigm shift, which aims at resolving our current system issues for modern workloads, is referred to as near-memory computing (NMC). 

%The rapid evolution of workloads has prompted researchers to gauge the capability of these applications in the context of NMC.
%Past works, such as \cite{7284059, hsieh2016accelerating, azarkhish2016design, 7551394, 7927081}, have efficiently applied NMC architectures for a wide range of applications%, from graph processing and databases to neural networks and bioinformatics.such as graph processing, databases, neural networks, and bionformatics.
NMC architectures have been efficiently applied in previous work for a wide range of applications such as graph processing, databases, neural networks, and bioinformatics \gagan{(cite all the works)}.
These distinct workloads, stretching across various domains, have made even more crucial that computer designers understand the characteristics of these emerging
applications to optimize these future systems for their target workloads. Additionally, NMC systems have mostly proven to be effective against memory-intensive applications and are hence tailored towards this kind of workloads. For HW mapping to a specific workload, it is critical to analyze the application to quantify the demand of various applications on the architecture design.

Traditionally, workload characterization has been done by profiling benchmarks using e.g. hardware performance counters. However, this technique is limited by the influence of micro-architecture features. To avoid this pitfall, in the past decade there has been a fair amount of research towards characterizing workloads in a micro-architecture independent way. The idea is to profile instruction traces and collect inherent application information such as operation mix, memory behavior, etc. This approach provides more relevant workload characteristics than by using hardware performance counters. In this scope, PISA \cite{Anghel2016}, a platform-independent software analysis tool was developed. PISA is capable of extracting results in a true micro-architecture agnostic manner, by utilizing Low Level Virtual Machine (LLVM)'s Intermediate Representation (IR). By following this approach, we can retrieve fundamental application proprieties and help in evaluating system performance bottlenecks. This framework can be easily applied for tuning of NMC architectures. Therefore, we extend the capabilities of PISA to extract characteristics directed towards NMC architectures.

% Nowadays Moore's Law \cite{moore} and Dennard Scaling \cite{Dennard1999DesignOI} have reached an end-point. This is due to performance per watt that are not doubling every 18 months and to the power that is not scaling how expected reducing the gate size. This difference between current and predicted performance is called \emph{Dark Silicon gap}.

% Furthermore, the improvements in memory and processor technology grew at different speeds, respectively around $7\%$ \cite{bookCA} and $80\%$ \cite{baskett}.
% This gap between this two technology is very critical to solve and it's called \emph{Memory Wall} by Wulf and McKee \cite{Wulf:1995:HMW:216585.216588}. McKee \cite{McKee:2004:RMW:977091.977115} in 2006 specified that not all the applications are affected by this problem. For instance, multimedia applications benefited from improvement in CPU performance. On the other hand scientific and commercial workloads shows a highly limitation due to memory bottlenecks. 

% In addition to that big data applications that uses an huge quantity of data and they cannot be performed on current HPC systems \cite{PHILIPCHEN2014314} are becoming widespread in different fields such as astronomy, graph processing, neural networks, etc.

% New approaches as Near-Memory Computing try to bring the computation close to data \cite{overviewpaper}, contrariwise to conventional systems in which data are moved through all the hierarchies. However they're missing specific tools for workload characterization focused on the memory and parallelism characteristic, that are critical for these kind of approaches. First profiling tools date 60's and during the years many analysis approach has been provided. Since Near Memory Computing systems are not well defined, at this stage is essential a characterization methodology that is target independent in order to understand the real intrinsic behavior of applications. We extend the current State-of-the-Art tool for platform independent analysis \cite{Anghel2015AnIA}, that supports the multi-threads and multi-process standards, with metrics focused on Memory and Parallelism behavior. 

The main contributions of this paper are:
\begin{itemize}

%\item We oveon workload characterization tools.%\todo[inline]{don't agree to it, we need to do it anyhow for the related work}
\item We present NMC specific micro-architecture independent application metrics.  
\item We extend state the of the art platform-independent software analysis tool called PISA with the NMC specific micro-architecture independent application metrics.
%\item Instruction-level parallelism specialization to estimate data-level parallelism. \todo[inline]{need to compared these metrics with already used metrics in NMC to see what additional information/benefit these metrics provide?}
%\item Metrics for basic-block level parallelism and for data parallel loop estimation.
%\item Analysis of previously presented metrics as spatial locality and memory entropy on a set of multi-threaded applications, \todo[inline]{why multi-threaded applications make the analysis new ?} highlighting whether the metrics are helpful for NMC and showing which application may benefit from this architecture. 
\item We propose a method to validate the relevance of proposed metrics in selecting the kernels to offload on NMC hardware.
\item We present prior art on workload characterization tools and position our work in the existing literature.%\todo[inline]{don't agree to it, we need to do it anyhow for the related work}


\end{itemize}


The rest of the paper is organized as follows: \emph{Section \ref{sec:backgrounds}} presents the LLVM framework and the tool architecture that we extended.
%The characterization metrics that we embedded into the tool are described in \emph{Section \ref{sec:metrics}}.
In \emph{Section \ref{sec:metrics}} we describe the characterization metrics we embedded into PISA.
The methodology is presented in \emph{Section \ref{sec:methodology}}. In \emph{Section \ref{sec:results}} we show and discuss the characterization results. We give an overview of the main research on workload characterization in general and from the NMC perspective in particular in \emph{Section \ref{sec:relatedworks}}. Finally, \emph{Section \ref{sec:conclusions}} concludes this paper.

%\raggedbottom

==> sections/metrics_OLD.tex <==
We extend the state-of-the-art tool for target-independent workload characterization called PISA. As mentioned, 
we integrate into this framework fundamental metrics for NMC systems. Especially, we focus on the intrinsic memory and parallelism behavior of the workloads. Memory behavior is essential to decide which part of the application should be offloaded to an NMC architecture. Parallelism is crucial to \gagan{determine}\gaganRemove{decide} if a specific parallel architecture should be integrated into an NMC system.

%its most important features are the target-independence and the possibility to analyze multi-threaded and multi-process applications. 

%We extended PISA, a target-independent tool for workload characterization, that support multi-threaded and multi-process applications, with metrics focused on the Memory and Parallelism. These metrics are explained in the following subsections.

\subsection{Memory entropy}
The first metric related to memory behavior that we added is the memory entropy. The memory entropy measures the randomness of the memory addresses accessed. If the memory entropy is high, which means a higher miss ratio, the application may benefit from 3D-stacked memory \gaganCheck{because of the volume of data moved from the main memory to the caches(EXPLAINATION IS NOT GOOD)}. In information theory, Shannon's formula \cite{6773263} is used to capture entropy \gaganCheck{(ENTROPY OF WHAT)}. We embed in PISA, the formula defined by Yen et al.~\cite{Yen:2008:NHT:1521747.1521793}. They applied Shannon's definition to memory addresses as shown below:

\begin{equation}
\textrm{Memory-entropy} = - \sum^{2^n}_{i=1}\hat{p}(x_i)log_2\hat{p}(x_i)
\label{eq:entropy1}
\end{equation}

In \emph{Equation \ref{eq:entropy1}}, $x_i$ is a n-bit random variable, $\hat{p}(x_i)$ is the occurrence probability for the value $x_i$ and $2^n$ is the number of values that $x_i$ can take. $\hat{p}(x_i)$ is defined by:

\begin{equation}
\begin{split}
\hat{p}(x_i)=\frac{1}{d}\sum^{d}_{j=1}I(a_j=x_i) \\
\textrm{where} \; I(a_j=x_i)=1 \; if \; (a_j=x_i), \\ 
0 \; \textrm{otherwise} \; \textrm{and} \; 0log0=0
\end{split}
\label{eq:entropy2}
\end{equation}

In \emph{Equation \ref{eq:entropy2}}, $d$ memory addresses are accessed during the execution and they are represented as $\{a_j\}^d_{j=1}$. Each address is in the range $[0,2^{n-1}]$, where $n$ is the length of the address in bits. If every address has the same occurrence probability the entropy is $n$; if only one address is accessed the entropy is $0$. Otherwise, the entropy is within $0$ and $n$. 
The memory entropy metrics does not distinguish whether the accesses contain sequential patterns or random accesses. Therefore we need additional metrics, like spatial locality.

\subsection{Data reuse distance for multiple cache-line size and spatial locality}
Data reuse distance or data temporal reuse (DTR) is a helpful metric to detect cache inefficiencies. The DTR of an address is the number of unique addresses accessed since the last reference of the requested data. 
This metric is present in the default framework. However, the tool can compute it only for a fixed cache line size, which represents the address granularity e.g. if the cache line is 16Bytes the 4 least significant bits (LSB) are discarded to compute unique address in the DTR computation. We modify the tool in order to compute the DTR for different cache line sizes. This extends the available analysis opportunities. For instance, we employed the DTR to compute the spatial locality.

%We extend the DTR computation and  compute it starting from the word size to the value selected by the user. This extends the available analysis opportunities. For instance, it enables us to estimate the L1 miss-ratio for an LRU cache, the number of external accesses, and the number of transferred bytes for different cache line sizes. In this way, it is feasible to determine the best cache and cache line size outlining an optimization problem. \\

%Spatial locality, which measures the probability of accessing nearby memory locations, can be derived from DTR.
We extend PISA with the spatial locality score inspired by Gu et al. \cite{Gu:2009:CMS:1542431.1542446}. The key idea behind this spatial locality score is to detect a reduction in DTR when doubling the cache line size. To estimate the spatial locality in a program two elements are fundamental: 1) histograms of data reuse distance for different cache line sizes, 2) distribution maps to keep track of changes in DTR for each access doubling the cache line size.
%\gagan{"FIRSTLY" MAKES SENSE??}Firstly, h
Histograms are used to compute the DTR distribution for different cache-line sizes. In \cite{Gu:2009:CMS:1542431.1542446} the reuse signature has been defined as a pair $<R,P>$, where $R$ is a series of consecutive DTR ranges of bins, represented as: $r_i=[d_i,d_{i+1})$. These bins are a logarithmic progression defined as:  $d_{i+1} = 2d_i (i \geq 0)$. $P$ is the distribution probabilities $p_i$ of the bin $r_i$. This reuse signature is used later to normalize the results.
The next step consists of building a distribution map. This map keeps track of each change in the DTR for every access. The distribution map has $i$ rows representing the bins using a cache line size $b$ and $j$ columns representing the bins using a doubled cache line size $2b$. Each cell is the probability $p_{ij}$ of the bin $i$ using a cache line size $b$ to change in a bin $j$ using a cache line size $2b$.  Differently from \cite{Gu:2009:CMS:1542431.1542446} we compute the sum of the cells in a row where $i<j$, as shown in \emph{Equation \ref{eq:slq}}. We do that because we want to express all the changes in data reuse distance. The spatial locality score for the bin $i$ is:

\begin{equation}
SLQ(i)=\sum_{j=0}^{j<i}p_{ij}
\label{eq:slq}
\end{equation}

To compute the spatial locality score related to a pair of cache line sizes $<b,2b>$ we first compute the absolute values of the weighted sum that uses the probabilities $p_i$ included in the reuse signature and then use the formula proposed by \cite{Gu:2009:CMS:1542431.1542446} to calculate the total score, which is the logarithmic weighted sum of absolute values:

\begin{equation}
SLQ=\frac{\sum_{\textrm{all} \; b}|\sum_{\textrm{all} \; i}SLQ^b(i)p_i^b|2^{-b}}{\sum_{\textrm{all} \; b}2^{-b}}
\label{eq:slqtotal}
\end{equation}

%\begin{equation}
%SLQ_b=\sum_{\textrm{all} \; i}SLQ^b(i)p_i^b
%\label{eq:slq2}
%\end{equation}

%The total spatial locality score is difficult to interpret because the weighting process gives more importance to lower cache line sizes pairs. 
The weighted score gives more importance to lower cache line sizes pairs.
Nevertheless, this can be interpreted as higher relevance of these lower pairs because bigger cache line sizes bring massive data transfers.

Applications with low spatial locality perform very bad on traditional systems with cache hierarchies because a small portion of data is utilized compared to the data loaded from the main memory to the caches. Thus these applications could benefit from NMC.% However, also workloads with high spatial locality could benefit from the larger bandwidth provided by the 3D-stacked memory in NMC systems. 

\subsection{Data-level parallelism}

Data-level parallelism (DLP) measures the average length of vector instructions that is used to optimize a program. DLP could be interesting for NMC when employing specific SIMD processing units in the logic layer of the 3D-stacked memory.



\begin{figure}[h]
\centering
\includegraphics[width=7.8cm,trim ={0 0.5cm 0 1.8cm},clip]{images/ilp_spec.eps}

\caption{The control flow graph (CFG) is commonly used to compute the ILP (as shown on the left). Also, CFG can be used to analyze ILP per type of instruction (as shown for memory instructions in the center). We further specialized this CFG to compute ILP per opcode (as shown for load instructions on the right). The ILP computed in this way represents how many instructions of the same opcode could run in parallel, which is referred to as data-level parallelism or DLP per instruction.\label{fig:ilpspecialized}}
\end{figure}

PISA can extract the instruction-level parallelism for all the instructions (see \emph{Figure \ref{fig:ilpspecialized}}, CFG on the left) and additionally per instruction category such as control, memory, etc. (see \emph{Figure \ref{fig:ilpspecialized}}, CFG in the center). As shown in the CFG on the right in \emph{Figure \ref{fig:ilpspecialized}}, we extract the ILP score per opcode and call it as $ ILP_{\textrm{specialized}, \textrm{opcode}}$ where opcode can be load, store, add, etc. This metric represents the number of instructions with the same opcode that could run in parallel. Next, we compute the weighted average (\emph{Equation \ref{eq:dlp}}) value for DLP using the weighted sum over all opcodes of $ ILP_{\textrm{specialized}, \textrm{opcode}}$.The weights are the frequency of the opcodes calculated by dividing the number of instructions per code with the number of instructions.

\begin{equation}
\begin{split}
DLP_{avg}=\sum_{\textrm{opcode}} ILP_{\textrm{specialized}, \textrm{opcode}} \frac{\#\textrm{instructions}_{\textrm{opcode}}}{\#\textrm{instructions}}
\end{split}
\label{eq:dlp}
\end{equation}

As the register allocation step is not performed at the level of intermediate representation, it is not possible to take into account the register consecutiveness in this score.
However, we want to show the optimization opportunities for compilers distinguishing between consecutiveness of load/store instruction addresses. We represent this with two scores: $DLP_1$ without address consecutiveness; $DLP_2$ with addresses consecutiveness into account. To compute them we use \emph{Equation \ref{eq:dlp}} changing the $ILP_{\textrm{specialized}, \textrm{opcode}}$ value for loads and stores.






\subsection{Basic-block level parallelism}

A basic-block is the smallest component in the LLVM's IR that can be considered as a potential parallelizable task. Basic-block level parallelism (BBLP) is an important metric for NMC because if it is high, then it is possible to exploit many processing units in the 3D-stacked memory logic layer. %However, also applications with a low level of parallelism can benefit from NMC approach by exploiting the high bandwidth coming from 3D-stacked memory technology.

To estimate BBLP in a workload, we developed a metric similar to ILP and DLP. The first assumption we made is to consider a basic-block as a set of instructions that can only be executed sequentially. Since loop index count could put an artificially tight constraint on the parallelism, we assume two different basic-block scheduling approaches (see \emph{Figure \ref{fig:bblpscheduling}}): 1) all the dependencies between basic-block are considered; 2) we consider a smart scheduling, assuming a compiler that can optimize loop index update dependencies. The difference between the two approaches can give an idea, as in the DLP case, of the optimization opportunities for compilers. We compute the two scores derived from the two scheduling options using the following formula (see \emph{Figure \ref{fig:bblpscheduling}}):

\begin{equation}
BBLP_{avg}=\frac{\# \textrm{instructions}}{\textrm{MaxIssueCycle}_{BBLP}}
\label{eq:bblp}
\end{equation}
Where $MaxIssueCycle_{BBLP}$ represents the cycle of the last executed instruction using the proposed scheduling approaches (red numbers in \emph{Figure \ref{fig:bblpscheduling}(b,c)}). $\#instructions$ represent the total number of instructions (see \emph{Figure \ref{fig:bblpscheduling}.a}).  

\begin{figure}[H]
\centering
\includegraphics[width=8.5cm,trim ={0 10.3cm 12.9cm 3.1cm},clip]{images/bblpscheduling.pdf}
\caption{BBLP/PBBLP methodology: a) example of LLVM dynamic trace; b) real scheduling for BBLP computation taking in account all dependencies; c) simplified scheduling for BBLP computation not taking in account dependencies such as loop index update (dependency between instruction 15-icmp and 17-getelementptr, see the numbers in a)); d) PBBLP values for each basic block (second and third block are a repeated basic block, since there is only a loop index dependecy, the PBBLP is equal to 2). %Furthermore, the second and the third basic blocks are two instances of the same basic block. Since they have only a dependency for loop index update, the PBBLP value is maximal and equal to 2.
\label{fig:bblpscheduling}}
\end{figure}


We also aim to estimate the presence of data parallel loops. Data parallel loops consists of basic-blocks that are repeated without any dependencies among their instances. A fast and straightforward estimation can be done by assigning a value to each basic-block between $1$ and the number of instances. When a basic-block has only one instance or all its instances have dependencies among them the score is $1$. Instead, when all its instances don't have dependencies among them the value is maximal and equal to the number of instances.\gagan{However} \gaganRemove{Contrariwise}, the score is within the range described above.
Other assumptions we made are: skip index update dependencies and omit basic-blocks that are used only for index update.



After assigning a score to each basic-block ($PBBLP_{BB}$),  we compute the weighted average value for PBBLP using the weighted sum (\emph{Equation \ref{eq:pbblp}}) over all scores ($PBBLP_{BB}$). The weights are the frequency of the basic-block instanes calculated by dividing the number of instances per basic-block with the number of total instances. 

\begin{equation}
PBBLP_{avg}=\sum_{BB}PBBLP_{BB}\frac{\#\textrm{instances}_{BB}}{\#\textrm{instances}_{\textrm{total}}}
\label{eq:pbblp}
\end{equation}
 
However, this score is only a speculative estimation that can show potential BBLP and consequently DLP, thus being less precise than the previously presented metrics.


==> sections/metrics_SCOPES.tex <==


In this section we summarize (see \emph{Table \ref{tab:newmetrics}}) the metrics we integrated into PISA~\cite{corda2019scopes}. 
Our work has been focused on the memory behaviour, which is essential to decide if an application should be accelerated with NMC architecture, and on the parallelism behaviour, which is crucial to decide if a specific parallel architecture should be integrated into an NMC system.

\begin{table}[H]
%\caption{Application parameters used for the evaluation on NMC and Host system}
\caption{Memory and Parallelism metrics}

\label{tab:newmetrics}
\centering
\scalebox{0.98}{
\begin{tabular}{l|l}
\hline
\multicolumn{2}{c}{\textbf{Metrics}}  \\ 
\hline
\textbf{Memory} & Memory Entropy\\
& Spatial Locality\\
\hline
\textbf{Parallelism} & Data-Level Parallelism\\
 & Basic-Block-Level Parallelism\\
 & Potential Basic-Block-Level Parallelism\\
 \hline
\end{tabular}
}
\end{table}

\subsection{Memory metrics}
We add memory entropy, which measures the randomness of the memory addresses accessed using an entropy formula adapted to the memory accesses. If the memory entropy is high, which means a higher cache miss ratio, the application may benefit from 3D-stacked memory because of the volume of data moved from the main memory to the caches.

Data reuse distance or data temporal reuse (DTR) is a helpful metric to detect cache inefficiencies. The DTR of an address is the number of unique addresses accessed since the last reference of the requested data. We integrate this metric into PISA for different cache line sizes in order to compute the Spatial locality metric.

Spatial locality measures the probability of accessing nearby memory locations.
The key idea behind this spatial locality score is to detect a reduction in DTR when doubling the cache line size. Usually, application with low spatial locality perform very bad on traditional systems with cache hierarchies because a small portion of data is utilized compared to the data loaded from the main memory to the caches

\subsection{Parallelism metrics}
Data-level parallelism (DLP) measures the average length of vector instructions that is used to optimize a program. DLP could be interesting for NMC when employing specific SIMD processing units in the logic layer of the 3D-stacked memory. We specialize the instruction-level parallelism (ILP) per opcode in order to estimate the DLP.

A basic-block is the smallest component in the LLVM's IR that can be considered as a potential parallelizable task. Basic-block level parallelism (BBLP) is a potential metric for NMC because it can estimate the task level parallelism in the application. The parallel tasks can be offloaded to multiple compute units located on the logic layer of a 3D-stacked memory. We develop a metrics similar to ILP considering the basic block as a set of instruction that can be run only sequentially.

We also aim to estimate the presence of data parallel loops. Data parallel loops consist of basic-blocks that are repeated without any dependencies among their instances. We develop a metric, PBBLP (Potential basic-block-level parallelism) that tries in a fast and straightforward manner to estimate the basic-block level parallelism in data parallel loops.

==> sections/metrics_SCOPES_old.tex <==


In this section we present the metrics we integrated into PISA. We %focused
focus on the memory behaviour, which is essential to decide if an application should be accelerated with a NMC architecture, and on the parallelism behaviour, which is crucial to decide if a specific parallel architecture should be integrated into an NMC system.

%We extend the state-of-the-art tool for target-independent workload characterization called PISA. As mentioned, 
%we integrate into this framework fundamental metrics for NMC systems. Especially, we focus on the intrinsic memory and parallelism behavior of the workloads. Memory behavior is essential to decide which part of the application should be offloaded to an NMC architecture. Parallelism is crucial to decide if a specific parallel architecture should be integrated into an NMC system.

%its most important features are the target-independence and the possibility to analyze multi-threaded and multi-process applications. 

%We extended PISA, a target-independent tool for workload characterization, that support multi-threaded and multi-process applications, with metrics focused on the Memory and Parallelism. These metrics are explained in the following subsections.


\subsection{Memory entropy}
The first metric related to memory behavior that we added is the memory entropy. The memory entropy measures the randomness of the memory addresses accessed. If the memory entropy is high, which means a higher cache miss ratio, the application may benefit from 3D-stacked memory because of the volume of data moved from the main memory to the caches. In information theory, Shannon's formula \cite{6773263} is used to capture entropy.

%
%\begin{equation}
%Entropy = - \sum^{N}_{i=1}p(x_i)log_2p(x_i)
%\label{eq:entropy}
%\end{equation}

%In Shannon's entropy $x$ (\emph{Equation \ref{eq:entropy}}) is the random variable, $p(x_i)$ is the occurrence probability for the value $x_i$ and $N$ is the number of values that $x$ can take. 
%\gagan{I WOULD WRITE IT THIS WAY\\}
%\gagan{where $x$ is the random variable, $p(x_i)$ is the occurrence probability for the value $x_i$ and $N$ is the number of values that $x$ can take.}

We embed in PISA, the formula defined by Yen et al. \cite{Yen:2008:NHT:1521747.1521793}. They applied Shannon's definition to memory addresses: $\textrm{Memory\_entropy} = - \sum^{2^n}_{i=1}\hat{p}(x_i)log_2\hat{p}(x_i)$, where $x_i$ is a n-bit random variable, $\hat{p}(x_i)$ is the occurrence probability for the value $x_i$ and $2^n$ is the number of values that $x_i$ can take. $\hat{p}(x_i)$ is defined by: $\hat{p}(x_i)=\frac{1}{d}\sum^{d}_{j=1}I(a_j=x_i)$ where $ I(a_j=x_i)=1 \; if \; (a_j=x_i), \; 0 \; \textrm{otherwise} \; \textrm{and} \; 0log0=0$.




%\begin{equation}
%\begin{split}
%\hat{p}(x_i)=\frac{1}{d}\sum^{d}_{j=1}I(a_j=x_i) \\
%\textrm{where} \; I(a_j=x_i)=1 \; if \; (a_j=x_i), \\ 
%0 \; \textrm{otherwise} \; \textrm{and} \; 0log0=0
%\end{split}
%\label{eq:entropy2}
%\end{equation}

%In \emph{Equation \ref{eq:entropy2}}, 
In the last formula the addresses are represented as  $\{a_j\}^d_{j=1}$, where $d$ is the number of different addresses accessed during the execution. Each address is in the range $[0,2^{n-1}]$, where $n$ is the length of the address in bits. If every address has the same occurrence probability the entropy is $n$; if only one address is accessed the entropy is $0$. Otherwise the entropy is within $0$ and $n$. The memory entropy metric does not distinguish whether the accesses contain sequential patterns or random accesses. Therefore we need additional metrics, like spatial locality.

\subsection{Data reuse distance for multiple cache-line size and spatial locality}
Data reuse distance or data temporal reuse (DTR) is a helpful metric to detect cache inefficiencies. The DTR of an address is the number of unique addresses accessed since the last reference of the requested data. 
This metric is present in the default framework. However, the tool could compute it only for a fixed cache line size, which represents the address granularity. We extend the DTR computation and compute it starting from the word size to the value selected by the user. This extends the available analysis opportunities e.g. we use it to compute the spatial locality metric. %For instance, this result has been used to implement the spatial locality metric. 

%For instance, it enables us to estimate the L1 miss-ratio for an LRU cache, the number of external accesses, and the number of transferred bytes for different cache line sizes. In this way, it is feasible to determine the best cache and cache line size outlining an optimization problem. \\

Spatial locality, which measures the probability of accessing nearby memory locations, can be derived from DTR. We extend PISA with the spatial locality score inspired by Gu et al. \cite{Gu:2009:CMS:1542431.1542446}. The key idea behind this spatial locality score is to detect a reduction in DTR when doubling the cache line size. To estimate the spatial locality in a program two elements are fundamental: 1) histograms of data reuse distance for different cache line sizes, 2) distribution maps to keep track of changes in DTR for each access doubling the cache line size.
%\gagan{"FIRSTLY" MAKES SENSE??}Firstly, h
Histograms are used to compute the DTR distribution probability for different cache-line sizes. In \cite{Gu:2009:CMS:1542431.1542446} the reuse signature has been defined as a pair $<R,P>$, where $R$ is a series of consecutive DTR ranges of bins, represented as: $r_i=[d_i,d_{i+1})$. These bins are a logarithmic progression defined as:  $d_{i+1} = 2d_i (i \geq 0)$. $P$ is the distribution probabilities $p_i$ of the bin $r_i$. This reuse signature is used later to normalize the results.
The next step consists of building a distribution map. This map keeps track of each change in the DTR for every access. The distribution map has $i$ rows representing the bins using a cache line size $b$ and $j$ columns representing the bins using a doubled cache line size $2b$. Each cell is the probability $p_{ij}$ of the bin $i$ using a cache line size $b$ to change in a bin $j$ using a cache line size $2b$.  Differently from \cite{Gu:2009:CMS:1542431.1542446} we compute the sum of the cells in a row where $i<j.\;$%,as shown in \emph{Equation \ref{eq:slq}}.
We do that because we want to express all the changes in data reuse distance. The spatial locality score for the bin $i$ is: $SLQ(i)=\sum_{j=0}^{j<i}p_{ij}$.
To compute the spatial locality score related to a pair of cache line sizes $<b,2b>$ we first compute the absolute values of the weighted sum that uses the probabilities $p_i$ included in the reuse signature and then use the formula proposed by \cite{Gu:2009:CMS:1542431.1542446} to calculate the total score, which is the logarithmic weighted sum of absolute values: $SLQ=\frac{\sum_{\textrm{all} \; b}|\sum_{\textrm{all} \; i}SLQ^b(i)p_i^b|2^{-b}}{\sum_{\textrm{all} \; b}2^{-b}}$.
The weighted score gives more importance to lower cache line sizes pairs.
Nevertheless, this can be interpreted as higher relevance of these lower pairs because bigger cache line sizes bring massive data transfers.
Usually, application with low spatial locality perform very bad on traditional systems with cache hierarchies because a small portion of data is utilized compared to the data loaded from the main memory to the caches.

%\begin{equation}
%SLQ(i)=\sum_{j=0, \; ..., \;j<i}p_{ij}
%\label{eq:slq}
%\end{equation}

%\begin{equation}
%SLQ=\frac{\sum_{\textrm{all} \; b}|\sum_{\textrm{all} \; i}SLQ^b(i)p_i^b|2^{-b}}{\sum_{\textrm{all} \; b}2^{-b}}
%\label{eq:slqtotal}
%\end{equation}

%Applications with low spatial locality perform very bad on traditional system with cache hierarchies because a small portion of data is utilized compared to the data loaded from the main memory to the caches. Thus these applications can benefit from NMC. However, also workloads with high spatial locality could benefit from the larger bandwidth provided by the 3D-stacked memory in NMC systems. 

\subsection{Data-level parallelism}
Data-level parallelism (DLP) measures the average length of vector instructions that is used to optimize a program. DLP could be interesting for NMC when employing specific SIMD processing units in the logic layer of the 3D-stacked memory. PISA can extract the instruction-level parallelism for all the instructions (see \emph{Figure \ref{fig:ilpspecialized}}, CFG on the left) and additionally per instruction category such as control, memory, etc. (see \emph{Figure \ref{fig:ilpspecialized}}, CFG in the center). As shown in the CFG on the right in \emph{Figure \ref{fig:ilpspecialized}}, we extract the ILP score per opcode and call it as $ ILP_{\textrm{specialized}, \textrm{opcode}}$ where opcode can be load, store, add, etc. This metric represents the number of instructions with the same opcode that could run in parallel. Next, we compute the weighted average value for DLP using the weighted sum over all opcodes of $ ILP_{\textrm{specialized}, \textrm{opcode}}$. The weights are the frequency of the opcodes calculated by dividing the number of instructions per code with the number of instructions.

$DLP_{avg}=\sum_{\textrm{opcode}} ILP_{\textrm{specialized}, \textrm{opcode}} \frac{\#\textrm{instructions}_{\textrm{opcode}}}{\#\textrm{instructions}}$ 

%that normalizes the DLP per opcode with the distribution probability of each opcode:\\ 

\begin{figure}[ht]
\centering
\includegraphics[width=7.8cm,trim ={0 0.5cm 0 1.8cm},clip]{images/ilp_spec.eps}

\caption{%The control flow graph (CFG) is commonly used to compute the ILP (as shown on the left).
Usually to compute ILP it has been used the control flow graph (CFG), left side.
The CFG in the center is used to compute the ILP per type of instructions. On the right our per opcode specialized CFG.\ahsan{try to reduce it to single line}\label{fig:ilpspecialized}}



%Also, CFG can be used to analyze ILP per type of instruction (as shown for memory instructions in the center). We further specialized this CFG to compute ILP per opcode (as shown for load instructions on the right). The ILP computed in this way represents how many instructions of the same opcode could run in parallel, which is referred to as data-level parallelism or DLP per instruction.\label{fig:ilpspecialized}}
\end{figure}

As the register allocation step is not performed at the level of intermediate representation, it is not possible to take into account the register consecutiveness in this score.
However, we want to show the optimization opportunities for compilers distinguishing between consecutiveness of load/store instruction addresses. We represent this with two scores: $DLP_1$ without address consecutiveness; $DLP_2$ with addresses consecutiveness into account. To compute them we use the previous formula changing the $ILP_{\textrm{specialized}, \textrm{opcode}}$ value for loads and stores.


%\begin{equation}
%\begin{split}
%DLP_{avg}=\sum_{\textrm{opcode}} DLP_{\textrm{opcode}} \frac{\#\textrm{instructions}_{\textrm{opcode}}}{\#\textrm{instructions}}\\
%\textrm{where} \; \; DLP_{\textrm{opcode}} \; = \; ILP_{\textrm{specialized}, \textrm{opcode}}
%\end{split}
%\label{eq:dlp}
%\end{equation}
\subsection{Basic-block level parallelism}

A basic-block is the smallest component in the LLVM's IR that can be considered as a potential parallelizable task. Basic-block level parallelism (BBLP) is a potential metric for NMC because it can estimate the task level parallelism in the application. The parallel tasks can be offloaded to multiple compute units located on the logic layer of a 3D-stacked memory.
%Basic-block level parallelism (BBLP) is an important metric for NMC because if it is high, then it is possible to exploit many processing units in the 3D-stacked memory logic layer. However, also applications with a low level of parallelism can benefit from NMC approach by exploiting the high bandwidth coming from 3D-stacked memory technology.
\begin{figure}[ht]
\centering
\includegraphics[width=8.5cm,trim ={0 10.3cm 12.9cm 3.1cm},clip]{images/bblpscheduling.pdf}
\caption{BBLP/PBBLP methodology: a) example of LLVM dynamic trace; b) real scheduling for BBLP computation taking in account all dependencies; c) simplified scheduling for BBLP computation not taking in account dependencies such as loop index update (in a) dependency between instruction 15 and 17); d) PBBLP values for each basic block (second and third block are a repeated basic block, since there is only a loop index dependecy, the PBBLP is equal to 2).\ahsan{try to reduce it to single line} %Furthermore, the second and the third basic blocks are two instances of the same basic block. Since they have only a dependency for loop index update, the PBBLP value is maximal and equal to 2.
\label{fig:bblpscheduling}}
\end{figure}
To estimate BBLP in a workload, we develop a metric similar to ILP and DLP. It is based on the assumption that  a basic-block, which is a set of instructions, can only be executed sequentially. Since loop index count could put an artificially tight constraint on the parallelism, we assume two different basic-block scheduling approaches (see \emph{Figure \ref{fig:bblpscheduling}}): 1) all the dependencies between basic-block are considered; 2) we consider a smart scheduling, assuming a compiler that can optimize loop index update dependencies. The difference between the two approaches can give an idea, as in the DLP case, of the optimization opportunities for compilers. We compute the two scores derived from the two scheduling options using the following formula: $BBLP_{avg}=\frac{\# \textrm{instructions}}{\textrm{MaxIssueCycle}_{BBLP}}$, where $MaxIssueCycle_{BBLP}$ represents the cycle of the last executed instruction using the proposed scheduling approaches (red numbers in \emph{Figure \ref{fig:bblpscheduling}.b,.c}). $\#instructions$ represent the total number of instructions (see \emph{Figure \ref{fig:bblpscheduling}.a}). 




We also aim to estimate the presence of data parallel loops. Data parallel loops consist of basic-blocks that are repeated without any dependencies among their instances. A fast and straightforward estimation can be done by assigning a value to each basic-block between $1$ and the number of instances. When a basic-block has only one instance or all its instances have dependencies among them the score is $1$. Instead, when all its instances don't have dependencies among them the value is maximal and equal to the number of instances. Contrariwise, the score is within the range described above.
Other assumptions we made are: skip index update dependencies and omit basic-blocks that are used only for index update.

After assigning a score to each basic-block ($PBBLP_{BB}$),  we compute the weighted average value for PBBLP using the weighted sum over all scores ($PBBLP_{BB}$). The weights are the frequency of the basic-block instances calculated by dividing the number of instances per basic-block with the number of total instances. $PBBLP_{avg}=\sum_{BB}PBBLP_{BB}\frac{\#\textrm{instances}_{BB}}{\#\textrm{instances}_{\textrm{total}}}$. Since this metric is an estimation we call it as potential basic-block level parallelism (PBBLP).

%\begin{equation}
%PBBLP_{avg}=\sum_{BB}PBBLP_{BB}\frac{\#\textrm{instances}_{BB}}{\#\textrm{instances}_{\textrm{total}}}
%\label{eq:pbblp}
%\end{equation}
 
%However, this score is only a speculative estimation that can show potential BBLP and consequently DLP, thus being less precise than the previously presented metrics.


==> sections/results_old.tex <==
%\begin{figure*}
%\centering
%\includegraphics[width=18cm]{images/entropy_polybenc}
%\caption{Memory Entropy analysis for PolyBench.
%\label{fig:entropypolybench}}
%\end{figure*}

\todo[inline]{This section should be fully re-written including assumptions (multi-threading, smaller dataset), new results for the application we simulated on NMC/P9, show first results using PCA}

We present a characterization of a set of selected applications from PolyBench and Rodinia benchmark. Then, we show the correlation between the added metrics to NMC performance.

\subsection{Dataset size and multi-threading}
    Few apps to show proportionality incresing dataset
    
     Rodinia apps to show similar values/behavior using single/multi-threading
     
     
\subsection{Characterization}
Entropy, locality parallelism

\subsection{Correlation with NMC performance}
PCA for added metrics for automatic extraction of the NMC kernels

\subsection{Other tools}
Vtune/perf characterization -> still issues in detecting good candidates




\color{blue}
We present a full characterization of the PolyBench suite for the added metrics and we show the multi-threaded capabilities of the tool with an example from the Rodinia benchmark.

%In this section we show and discuss the results extracted by the characterization tool. First we show the characterization for the added metrics for PolyBench and then we present the analysis on multi-threded applications as Rodinia.

%\subsection{Educational Example}
%\color{red} AN EXAMPLE THAT SHOULD BE FULL EXPLAINED AND UNDERSTOOD --> e.g. MATRIX MULTIPLICATION \color{black}

\subsection{PolyBench}
Our primary goal is to show the suitability of the added metrics for NMC and highlight those applications that can benefit from these kinds of systems. We did not include \emph{nussinov} and \emph{floyd-wharshall} into the memory characterization because they are the only two integer applications. This is a problem in the spatial locality computation because otherwise, the smallest location accessed by the programs will be different: 4Bytes for integer applications whereas 8Bytes for the floating point ones.


\emph{Figure \ref{fig:entropypolybench}} presents the memory-entropy analysis. This metric is strictly related to the dimension of the address space accessed by the workload. We also plot memory-entropy changes at different granularity cutting the least-significant bits (LSBs) of the address to represent larger data access granularity. This score is quite similar for all the analyzed application using similar data-sets. Only few of them as \emph{durbin} and \emph{jacobi-1d} have a lower value. Moreover, these two applications don't show changes of entropy when cutting the higher LSBs. We also highlight how only a few applications have a lower level of entropy than the others. Hence, these applications can benefit less from NMC architectures than the others.

\begin{figure}[H]
\centering
\includegraphics[width=8cm]{images/entropypollyhalf}
\caption{Memory entropy analysis for PolyBench.
\label{fig:entropypolybench}}
\end{figure}





\begin{figure*}
\centering
\includegraphics[width=17.05cm]{images/spatiallocalitypolybench}
\caption{Spatial locality analysis for PolyBench.
\label{fig:spatiallocalitypolybench}}
\end{figure*}

 \begin{figure*}
\centering
\includegraphics[width=17.3cm]{images/parallelismpolybench}
\caption{PolyBench parallelism characterization.
\label{fig:parallelismpolybench}}
\end{figure*}

Related to memory behavior, we show in \emph{Figure \ref{fig:spatiallocalitypolybench}} the spatial locality characterization for these workloads. As expected, we can distinguish different behaviors among the benchmarks. \emph{Durbin} shows an interesting behavior with low entropy and high spatial locality. This application is probably not a good candidate for NMC because it uses a small address space with high locality. The total score for spatial locality adopted is not easy to utilize to quantify the spatial locality for each application. This is due to the normalization in \emph{Equation \ref{eq:slqtotal}}. For instance, the \emph{gramschmidt} total score is very low. On the other hand, it has high spatial locality when doubling the cache-line size from $256B$ to $512B$. This can be interpreted as cost-ineffective when doubling large cache line size. Matrix multiplication and stencil algorithms show, as expected, higher levels of spatial locality. On the other hand algorithms such as \emph{deriche} and \emph{correlation} show a lower level of spatial locality, in this case, it is also possible to notice that \emph{deriche} has a considerable space of addresses, from the memory-entropy characterization. 
Since the spatial locality results for most of the applications are far from the maximum, that is 1, then many of them could benefit from new 3D stacking memory technologies used in NMC systems. 
%Since the spatial locality maximum can be 1 and many of these workloads show low spatial locality level, then they could benefit from new 3D stacking memory technologies used in NMC systems.
However, applications with high spatial locality could also benefit from NMC mostly when increasing the data-set and consequently moving more data off-chip.\\
Results collected for the parallelism characterization in PolyBench are presented in \emph{Figure \ref{fig:parallelismpolybench}}. As expected for the data-level parallelism analysis matrix multiplications based algorithms show the highest values. Moreover, the difference between the two DLP scores proposed seems to be very limited. Only small variation can be noticed, for instance between \emph{trmm} and \emph{syrk}. Here, the difference is due to load/store with non-sequential accesses and could be improved by compiler exploiting data mapping techniques. Instead the BBLP scores shows significant differences for few application such as \emph{deriche}, \emph{nussinov}, \emph{symm} and \emph{floyd-warshall}. These results highlight possible parallelism optimizations that can be performed by compilers. 
It can be seen that the basic-block level parallelism is, as expected in the Berkeley dwarf \cite{Asanović:EECS-2006-183}, high for the matrix-based algorithm and low, for instance, in the \emph{fdtd-2d} workload.
Finally, the $PBBLP$ score tries to highlight the presence of the data parallel loop and can give an estimation of how much parallelism can be achieved using vectorization or loop unrolling strategies.
High level of parallelism could help in NMC exploiting the logic layer interfaced with parallel and SIMD architectures on top of the 3D stacked memory.




\subsection{Rodinia}
We characterize a set of Rodinia applications using the added metrics to show the multi-threaded capabilities of PISA.

For instance, \emph{Figure \ref{fig:localityrodinia}} shows the spatial locality analysis for the selected workloads from Rodinia. In particular, it can be noticed that the average values of this metric are quite constant when increasing the number of threads. The variability per-thread, represented by the standard deviation from the mean value, is low, except for \emph{nn}. This low variability is due to the master thread that has a higher overhead from other threads.




Briefly, as for spatial locality, we analyzed the master-thread variability for the other metrics.
We must mention that, similar to Polybench results, the parallelism level for these applications is high, except for \emph{lud}. This result shows possible opportunities for compiler-level optimization and, as previously mentioned, benefits from NMC approach. However, as expected the level of parallelism decreases with an increase in the number of threads.

\begin{figure}[H]
\centering
\includegraphics[width=7.5cm]{images/spatiallocalityrodinia}
\caption{Spatial locality analysis for Rodinia.
\label{fig:localityrodinia}}
\end{figure}


%This result is similar to the one obtained in the PolyBench characterization and it means that further optimizations at compiler lee are possible and that many of them can benefit from the NMC approach. 

\color{black}
